Chest X-rays Classification: A Multi-Label and Fine-Grained Problem

The widely used ChestX-ray14 dataset addresses an important medical image classification problem and has the following caveats: 1) many lung pathologies are visually similar, 2) a variant of diseases including lung cancer, tuberculosis, and pneumonia are present in a single scan, i.e. multiple labels and 3) The incidence of healthy images is much larger than diseased samples, creating imbalanced data. These properties are common in medical domain. Existing literature uses stateof- the-art DensetNet/Resnet models being transfer learned where output neurons of the networks are trained for individual diseases to cater for multiple diseases labels in each image. However, most of them don't consider relationship between multiple classes. In this work we have proposed a novel error function, Multi-label Softmax Loss (MSML), to specifically address the properties of multiple labels and imbalanced data. Moreover, we have designed deep network architecture based on fine-grained classification concept that incorporates MSML. We have evaluated our proposed method on various network backbones and showed consistent performance improvements of AUC-ROC scores on the ChestX-ray14 dataset. The proposed error function provides a new method to gain improved performance across wider medical datasets.

==> contrib/supply.tex <==
%\section{Supplementary}
%\label{sec:supply}

\section{Dataset}
\label{sec:su-data}
\vspace*{-2.0cm}

Table~\ref{table:class} presents 15 different disease types for skin lesion. The ``Presence'' column shows the percentage of images from every disease category in the dataset.

\begin{table}
\centering 
\caption{}
\scalebox{1.0}

	\begin{tabular}{lcc}
	\hline
	\hline
	{\bf Disease} & {\bf Presence (percent)} \\	
	\hline
	\hline
	Melanoma & 4.6\% \\	
	Basal Cell Carcinoma & 20.0\% \\
	Squamous Cell Carcinoma & 2.9\% \\
	Actinic Keratosis & 25.4\% \\
	Blue naevus & 1.0\% \\
	Bowens disease & 2.4\% \\
	Compound naevus & 7.7\% \\
	Dermal naevus & 1.6\% \\
	Dermatofibroma & 2.8\% \\
	Hemangioma & 1.2\% \\
	Junctional naevus & 2.4\% \\
	Keratotic lesion & 2.8\% \\
	Seborrheic keratosis & 20.4\% \\
	Sebaceous hyperplasia  & 1.3\% \\
	Solar lentigo & 3.5\% \\
	\hline
	\end{tabular}
\label{table:class}
\end{table} 

%\pagebreak

\begin{figure}
	\centering
	\begin{minipage}{0.8\columnwidth}
	\centering
	\includegraphics[width=0.16\columnwidth]{./pic/39-1.jpg}
	\includegraphics[width=0.16\columnwidth]{./pic/43-1.jpg}
	\includegraphics[width=0.16\columnwidth]{./pic/83-1}
	\includegraphics[width=0.16\columnwidth]{./pic/142-1}
	\includegraphics[width=0.16\columnwidth]{./pic/72-1}
	\end{minipage}
	~
    \begin{minipage}{0.8\columnwidth}
	\centering
	\includegraphics[width=0.16\columnwidth]{./pic/39-2.jpg}
	\includegraphics[width=0.16\columnwidth]{./pic/43-2.jpg}
	\includegraphics[width=0.16\columnwidth]{./pic/83-2}
	\includegraphics[width=0.16\columnwidth]{./pic/142-2.jpg}
	\includegraphics[width=0.16\columnwidth]{./pic/72-2}
	\end{minipage}
\caption{Figure shows ``Clinical''(upper row) vs ``Dermoscopic''(lower row) over the same lesion.}
\label{pic:image}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{./pic/15}
\caption{Samples of the 15 skin disease lesion. For each lesion, we show the boundary of CAM-BP activation map.}
\label{pic:15}
\end{figure}

\pagebreak

\section{Network Structure}
\vspace*{-12cm}


\textbf{Sole-Net} and \textbf{Share-Net} architectures are shown in Table.~\ref{table:archi}.
\textbf{Triple-Net} architecture is presented in Table.~\ref{table:archi-2}.

\vspace*{-2.5cm}


\label{sec:su-net}
\begin{table}
\centering 
\caption{\small{Sole-Net and Share-Net Architecture}}
	\begin{tabular}{lcccccc}
	{\bf Layer-name}&{\bf Layer-type}&{\bf Kernel}&{\bf Stride/Pad}&{\bf Filters}&{\bf Activation} \\	
	\hline
	$C_{C/D_{1}}$ & Convolution & (3,3) & 1/1 & 64 & ReLu \\	
	$C_{C/D_{2}}$ & Convolution & (3,3) & 1/1 & 64 & ReLu \\	
	$C_{C/D_{3}}$ & Max Pooling & (2,2) & 2/0 & - & - \\
	$C_{C/D_{4}}$ & Convolution & (3,3) & 1/1 & 128 & ReLu \\	
	$C_{C/D_{5}}$ & Convolution & (3,3) & 1/1 & 128 & ReLu \\	
	$C_{C/D_{6}}$ & Max Pooling & (2,2) & 2/0 & - & - \\
	$C_{C/D_{7}}$ & Convolution & (3,3) & 1/1 & 256 & ReLu \\	
	$C_{C/D_{8}}$ & Convolution & (3,3) & 1/1 & 256 & ReLu \\	
	$C_{C/D_{9}}$ & Convolution & (3,3) & 1/1 & 256 & ReLu \\	
	$C_{C/D_{10}}$ & Max Pooling & (2,2) & 2/0 & - & - \\
	$C_{C/D_{11}}$ & Convolution & (3,3) & 1/1 & 512 & ReLu \\	
	$C_{C/D_{12}}$ & Convolution & (3,3) & 1/1 & 512 & ReLu \\	
	$C_{C/D_{13}}$ & Convolution & (3,3) & 1/1 & 512 & ReLu \\
	$C_{C/D_{14}}$ & Max Pooling & (2,2) & 2/0 & - & - \\	
	$C_{C/D_{15}}$ & Convolution & (3,3) & 1/1 & 512 & ReLu \\	
	$C_{C/D_{16}}$ & Convolution & (3,3) & 1/1 & 512 & ReLu \\	
	$C_{C/D_{17}}$ & Convolution & (3,3) & 1/1 & 512 & ReLu \\
	$C_{C/D_{18}}$ & Max Pooling & (2,2) & 2/0 & - & - \\
	$C_{C/D_{19}}$ & Fully-Connected & - & - & 4096 & Relu \\
	$C_{C/D_{20}}$ & Dropout & 0.5 ratio & - & - & - \\
	$C_{C/D_{21}}$ & Fully-Connected & - & - & 4096 & Relu \\
	$C_{C/D_{22}}$ & Dropout & 0.5 ratio & - & - & - \\
	$C_{C_{23}}$ & Classifier Clinical & - & - & - & - \\
	$C_{D_{23}}$ & Classifier Dermoscopic & - & - & - & - \\
	$C_{1}$ & Eltwise-sum & - & - & - & Avg \\
	\hline
	\end{tabular}
	\label{table:archi}
\end{table}

\begin{table}
\centering 
\caption{\small{Triplet-Net Architecture}}
	\begin{tabular}{lcccccc}
	{\bf Layer-name}&{\bf Layer-type}&{\bf Kernel}&{\bf Stride/Pad}&{\bf Filters}&{\bf Activation} \\	
	\hline
	$C_{C/D_{1}}$ & Convolution & (3,3) & 1/1 & 64 & ReLu \\	
	$C_{C/D_{2}}$ & Convolution & (3,3) & 1/1 & 64 & ReLu \\	
	$C_{C/D_{3}}$ & Max Pooling & (2,2) & 2/0 & - & - \\
	$C_{C/D_{4}}$ & Convolution & (3,3) & 1/1 & 128 & ReLu \\	
	$C_{C/D_{5}}$ & Convolution & (3,3) & 1/1 & 128 & ReLu \\	
	$C_{C/D_{6}}$ & Max Pooling & (2,2) & 2/0 & - & - \\
	$C_{C/D_{7}}$ & Convolution & (3,3) & 1/1 & 256 & ReLu \\	
	$C_{C/D_{8}}$ & Convolution & (3,3) & 1/1 & 256 & ReLu \\	
	$C_{C/D_{9}}$ & Convolution & (3,3) & 1/1 & 256 & ReLu \\	
	$C_{C/D_{10}}$ & Max Pooling & (2,2) & 2/0 & - & - \\
	$C_{C/D_{11}}$ & Convolution & (3,3) & 1/1 & 512 & ReLu \\	
	$C_{C/D_{12}}$ & Convolution & (3,3) & 1/1 & 512 & ReLu \\	
	$C_{C/D_{13}}$ & Convolution & (3,3) & 1/1 & 512 & ReLu \\
	$C_{C/D_{14}}$ & Max Pooling & (2,2) & 2/0 & - & - \\	
	$C_{C/D_{15}}$ & Convolution & (3,3) & 1/1 & 512 & ReLu \\	
	$C_{C/D_{16}}$ & Convolution & (3,3) & 1/1 & 512 & ReLu \\	
	$C_{C/D_{17}}$ & Convolution & (3,3) & 1/1 & 512 & ReLu \\
	$C_{C/D_{18}}$ & Max Pooling & (2,2) & 2/0 & - & - \\
	$C_{C/D_{19}}$ & Fully-Connected & - & - & 4096 & Relu \\
	$C_{C/D_{20}}$ & Dropout & 0.5 ratio & - & - & - \\
	$C_{C/D_{21}}$ & Fully-Connected & - & - & 4096 & Relu \\
	$C_{C/D_{22}}$ & Dropout & 0.5 ratio & - & - & - \\
	$C_{C_{23}}$ & Classifier-Cli & - & - & - & - \\
	$C_{D_{23}}$ & Classifier-Der & - & - & - & - \\
	$C_{T_{1}}$	   & Concatenation & -   & -   & - & - \\	
	$C_{T_{2}}$ & Convolution & (3,3) & 1/1 & 512 & (ReLu,BatchNorm) \\	
	$C_{T_{3}}$ & Convolution & (3,3) & 1/1 & 512 & (ReLu,BatchNorm) \\	
	$C_{T_{4}}$ & Convolution & (3,3) & 1/1 & 512 & (ReLu,BatchNorm) \\
	$C_{T_{5}}$ & Max Pooling & (2,2) & 2/0 & - & - \\	
	$C_{T_{6}}$ & Fully-Connected & - & - & 4096 & Relu \\
	$C_{T_{7}}$ & Dropout & 0.5 ratio & - & - & - \\
	$C_{T_{8}}$ & Fully-Connected & - & - & 4096 & Relu \\
	$C_{T_{9}}$ & Dropout & 0.5 ratio & - & - & - \\
	$C_{T_{10}}$ & Classifier-(Cli,Der) & - & - & - & - \\
	\hline
	\end{tabular}
	\label{table:archi-2}
\end{table}

\pagebreak


\section{Confusion Matrix}
\label{sec:conf}
\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{./pic/confusion_matrix}
\caption{The above figure shows normalised confusion matrix produced by Triplet-net CAM-BP on 15 skin disease classification task. The disease type 1 to 15 follows the same order as in Table.~\ref{table:class}.}
\label{pic:15}
\end{figure}
